MACAROON: Training Vision-Language Models To Be Your Engaged Partners

Large vision-language models (LVLMs), while proficient in following instructions and responding to diverse questions, invariably generate detailed responses even when questions are ambiguous or unanswerable, leading to hallucinations and bias issues. Thus, it is essential for LVLMs to proactively engage with humans to ask for clarifications or additional information for better responses. In this study, we aim to shift LVLMs from passive answer providers to proactive engaged partners. We begin by establishing a three-tiered hierarchy for questions of invalid, ambiguous, and personalizable nature to measure the proactive engagement capabilities of LVLMs. Utilizing this hierarchy, we create PIE, (ProactIve Engagement Evaluation) through GPT-4o and human annotators, consisting of 853 questions across six distinct, fine-grained question types that are verified by human annotators and accompanied with well-defined metrics. Our evaluations on \benchmark indicate poor performance of existing LVLMs, with the best-performing open-weights model only achieving an Aggregate Align Rate (AAR) of 0.28. In response, we introduce MACAROON, self-iMaginAtion for ContrAstive pReference OptimizatiON, which instructs LVLMs to autonomously generate contrastive response pairs for unlabeled questions given the task description and human-crafted criteria. Then, the self-imagined data is formatted for conditional reinforcement learning. Experimental results show MACAROON effectively improves LVLMs' capabilities to be proactively engaged (0.84 AAR) while maintaining comparable performance on general tasks.

==> contents/00_abstract_old.tex <==
\begin{abstract}

% While LVLMs demonstrate strong performance in following instructions and answer questions, 
% \ew{I feel like we don't have to say the `while...' part, just ``When facing unanswerable or ambiguous questions, LVLMs may invariably...''} 
When facing unanswerable or ambiguous questions, 
large vision-language models (LVLMs) may invariably provide detailed responses, resulting in hallucination and bias issues. 
% 
% Specifically, they may invariably provide detailed responses even in face of unanswerable or ambiguous human questions, resulting in hallucination and bias issues.
% 
% or convey an illusion of thorough understanding, despite often lacking genuine knowledge of the posed question. 
% benchmark construction
In such cases, it is essential for LVLMs to proactively engage with users to ask for clarifications or additional information to help them answer the question. 
In this study, we aim to shift LVLMs from passive answer providers to proactive engaged partners.
We begin by establishing a three-tiered \heng{not sure what three-tiered means} question hierarchy to measure the stepwise proactive engagement capabilities of LVLMs.
% Describe the benchmark
Utilizing this hierarchy, \heng{what taxonomy? elaborate three questions} we create \img{figures/pie2.pdf}\textbf{\benchmark} (\textbf{P}roact\textbf{I}ve \textbf{E}ngagement Evaluation), which consists of 853 questions across six distinct and fine-grained question types, such as unanswerable, subject ambiguity, and latent human preferences questions. Each type of questions is verified by human annotators and accompanied with well-defined metrics. 
% Evaluation 
Our evaluations on \benchmark indicate poor performance of existing LVLMs, with the best-performing open-weights model only achieving an Aggregate Align Rate of 0.23.
% Our approach
In response, we introduce \img{figures/macaroon4.pdf}\textbf{\approach}, self-i\textbf{M}agin\textbf{A}tion for \textbf{C}ontr\textbf{A}stive p\textbf{R}eference \textbf{O}ptimizati\textbf{ON}, which functions by instructing LVLMs to self-generate contrastive response pairs for unlabeled questions generated by GPT-4o given the task description and human-crafted criteria. 
% 
% \shujin{add our approach description to utilize the data.}
Then the self-imagined data is formatted for conditional reinforcement learning.
% 
% an interactive model designed to proactively engage by asking clarifying questions when faced with ambiguous user queries, challenge the false premises embedded in the given question, or even elicit human preferences to deliver more user-tailored responses. This was achieved by implementing Direct Preference Optimization (DPO) for reinforcement learning with preference data generated by self-imagination. 
% 
Experimental results show \approach can effectively improve LVLMs' capabilities to be proactively engaged while maintaining comparable performance on general tasks\footnote{The code will be made public.}. 
% \ew{We can put this in the footnote. In general, I feel like the abstract is a little long.}
\end{abstract}

==> contents/04_task.tex <==


\section{Task Formulation}
